Constraining Ongoing Volcanic Outgassing Rates and Interior Compositions of Extrasolar Planets with Mass Measurements of Plasma Tori

We present a novel method of constraining volcanic activity on extrasolar terrestrial worlds via characterization of circumstellar plasma tori. Our work generalizes the physics of the Io plasma torus to propose a hypothetical circumstellar plasma torus generated by exoplanetary volcanism. The quasi-steady torus mass is determined by a balance between material injection and ejection rates from volcanic activity and corotating magnetospheric convection, respectively. By estimating the Alfv\'en surfaces of planet-hosting stars, we calculate the torus mass-removal timescale for a number of exoplanets with properties amenable to plasma torus construction. Assuming a uniform toroidal geometry comparable to Io's "warm" torus, we calculate quasi-steady torus masses inferable from the optical depth of atomic spectral features in torus-contaminated stellar spectra. The calculated quasi-steady masses can be used to constrain the volcanic outgassing rates of each species detected in the torus, providing quantitative estimates of bulk volcanic activity and interior composition with minimal assumptions. Such insight into the interior state of an exoplanet is otherwise accessible only after destruction via tidal forces. We demonstrate the feasibility of our method by showcasing known exoplanets which are susceptible to tidal heating and could generate readily-detectable tori with realistic outgassing rates of order 1 ton s$^{-1}$, comparable to the Io plasma torus mass injection rate. This methodology may be applied to stellar spectra measured with ultraviolet instruments with sufficient resolution to detect atomic lines and sensitivity to recover the ultraviolet continuum of GKM dwarf stars. This further motivates the need for ultraviolet instrumentation above Earth's atmosphere.

==> table.tex <==
GJ 367 b & 0.007 & 0.035$^{+0.017}_{-0.012}$ & 3.43 & 44252 & 0.322 & 0.060$^{+0.070}_{-0.040}$ & 0.699 & 1368 & 0.46 & 0.46 & 51.30 & 10.153 & 9 & 5.91E+30 & 162$^{+194}_{-89}$ & RV; [1]\\ 
TOI-238 b & 0.021 & 0.060$^{+0.036}_{-0.021}$ & 1.78 & 867 & 1.273 & $<$0.180 & 1.402 & 1432 & 0.79 & 0.73 & 26.00 & 10.748 & 81 & 1.78E+30 & 27$^{+42}_{-16}$ & RV; [2]\\ 
GJ 9827 b & 0.019 & 0.045$^{+0.026}_{-0.015}$ & 1.79 & 1374 & 1.209 & $<$0.063 & 1.577 & 1173 & 0.61 & 0.60 & 28.90 & 10.370 & 30 & 5.10E+29 & 22$^{+32}_{-12}$ & RV; [3]\\ 
LHS 1678 b & 0.012 & 0.018$^{+0.013}_{-0.007}$ & 3.41 & 1516 & 0.860 & 0.033$^{+0.035}_{-0.023}$ & 0.685 & 869 & 0.34 & 0.33 & 64.00 & 12.600 & 20 & 1.19E+28 & 18$^{+35}_{-12}$ & RV; [4]\\ 
L 168-9 b & 0.021 & 0.042$^{+0.020}_{-0.016}$ & 1.69 & 1863 & 1.401 & $<$0.210 & 1.390 & 982 & 0.62 & 0.60 & 29.80 & 11.005 & 25 & 1.44E+30 & 16$^{+19}_{-10}$ & RV; [5]\\ 
K2-36 b & 0.023 & 0.060$^{+0.040}_{-0.021}$ & 1.13 & 549 & 1.423 & $<$0.093 & 1.430 & 1330 & 0.79 & 0.72 & 17.13 & 11.726 & 110 & 3.02E+29 & 15$^{+27}_{-9}$ & RV; [3]\\ 
HD 23472 d & 0.043 & 0.064$^{+0.033}_{-0.023}$ & 2.20 & 138 & 3.977 & 0.070$^{+0.050}_{-0.047}$ & 0.750 & 918 & 0.67 & 0.71 & 40.10 & 9.730 & 39 & 3.98E+25 & 12$^{+15}_{-7}$ & RV; [6]\\ 
GJ 486 b & 0.017 & 0.019$^{+0.011}_{-0.007}$ & 2.37 & 270 & 1.467 & 0.001$^{+0.002}_{-0.000}$ & 1.289 & 691 & 0.31 & 0.32 & 49.90 & 11.390 & 8 & 1.32E+25 & 8$^{+12}_{-5}$ & T; [7], [8]\\ 
HD 260655 b & 0.029 & 0.033$^{+0.014}_{-0.010}$ & 1.81 & 100 & 2.770 & 0.039$^{+0.043}_{-0.023}$ & 1.240 & 710 & 0.44 & 0.44 & 37.50 & 9.630 & 10 & 9.30E+26 & 6$^{+6}_{-3}$ & RV; [9]\\ 
Kepler-102 b & 0.055 & 0.070$^{+0.038}_{-0.025}$ & 1.48 & 11 & 5.287 & $<$0.100 & 0.460 & 855 & 0.80 & 0.72 & 27.95 & 12.072 & 108 & 1.70E+24 & 6$^{+8}_{-3}$ & RV; [3]\\ 
GJ 9827 c & 0.039 & 0.045$^{+0.026}_{-0.015}$ & 1.49 & 70 & 3.648 & $<$0.094 & 1.241 & 812 & 0.61 & 0.60 & 28.90 & 10.370 & 30 & 1.37E+27 & 5$^{+7}_{-3}$ & RV; [3]\\ 
Kepler-102 c & 0.067 & 0.070$^{+0.038}_{-0.025}$ & 1.41 & 6 & 7.071 & $<$0.094 & 0.567 & 776 & 0.80 & 0.72 & 27.95 & 12.072 & 108 & 9.96E+23 & 4$^{+5}_{-2}$ & RV; [3]\\ 
HD 63433 d & 0.050 & 0.091$^{+0.044}_{-0.032}$ & 0.40 & 58 & 4.209 & 0.160$^{+0.360}_{-0.120}$ & 1.073 & 1167 & 0.99 & 0.91 & 6.40 & 6.920 & 22 & 9.37E+26 & 3$^{+3}_{-2}$ & T; [10]\\ 
\hline
\multicolumn{17}{p{1.1\textwidth}}{\small{\textbf{Notes. }The table shows orbit semimajor axis $a$, Alfv\'en radius $R_A$, torus scale radius $H$, radiation magnetic confinement parameter $\zeta$, orbital period $P_{\rm Orb}$, eccentricity $e$, planetary radius $R_{\rm P}$, planetary equilibrium temperature $T_{eq}$, stellar mass $M_*$, stellar radius $R_*$, stellar rotation period $P_*$, magnitude $V$, system distance $D$, tidal heating $\dot{E}_{\rm heat}/\Im(\tilde{k}_2)$, and magnetospheric convection timescale $\tau$. The value of $H$ presented corresponds to a sulfur particle of mass $m=32$~amu; lighter (heavier) particles will have higher (lower) values of $H$. Note that the value listed $\dot{E}_{\rm heat}/\Im(\tilde{k}_2)$ corresponds to the case of $\Im(\tilde{k}_2)=1$. For reference the tidal heating of Io is $\simeq1.6\times10^{21}/\Im(\tilde{k}_2)$ ~erg~s$^{-1}$. References for $e$ and identification method (RV = radial velocity or radial velocity + transit fits; T = transit fits)  provided in the last column are: [1] \cite{Goffo2023ApJ...955L...3G}, [2] \cite{Suarez2024AA...685A..56S}, [3] \cite{Bonomo2023AA...677A..33B}, [4] \cite{Silverstein2024AJ....167..255S}, [5] \cite{ADef2020AA...636A..58A}, [6] \cite{Barros2022AA...665A.154B}, [7] \cite{WeinerMansfield2024ApJ...975L..22W}, [8] \cite{Caballero2022AA...665A.120C}, [9] \cite{Luque2022AA...664A.199L}, and [10] \cite{Capistrant2024AJ....167...54C}.}}

==> table2.tex <==
GJ 367 b & 0.7 & 0.7 & 2.6 & 1.4 & 0.9 & 16 & 26 & 1.9 & 51 & 715 \\ 
TOI-238 b & 17 & 17 & 64 & 34 & 22 & 396 & 639 & 46 & 1235 & 2898 \\ 
GJ 9827 b & 15 & 15 & 56 & 30 & 19 & 352 & 569 & 41 & 1098 & 2084 \\ 
LHS 1678 b & 6.3 & 6.5 & 24 & 13 & 8.1 & 150 & 241 & 18 & 466 & 732 \\ 
L 168-9 b & 22 & 23 & 86 & 46 & 29 & 535 & 864 & 63 & 1668 & 2275 \\ 
K2-36 b & 31 & 32 & 117 & 63 & 40 & 730 & 1178 & 86 & 2275 & 3035 \\ 
HD 23472 d & 70 & 72 & 266 & 143 & 90 & 1657 & 2675 & 194 & 5166 & 5142 \\ 
GJ 486 b & 18 & 18 & 67 & 36 & 23 & 418 & 674 & 49 & 1301 & 936 \\ 
HD 260655 b & 55 & 57 & 211 & 114 & 71 & 1316 & 2124 & 154 & 4102 & 2154 \\ 
Kepler-102 b & 177 & 183 & 674 & 363 & 228 & 4206 & 6788 & 493 & 13112 & 6553 \\ 
GJ 9827 c & 122 & 127 & 465 & 251 & 158 & 2902 & 4685 & 340 & 9049 & 3938 \\ 
Kepler-102 c & 311 & 323 & 1188 & 640 & 402 & 7412 & 11964 & 869 & 11147 & 7838 \\ 
HD 63433 d & 445 & 462 & 1697 & 914 & 575 & 10585 & 17086 & 1242 & 5333 & 7790 \\
\hline
\multicolumn{11}{p{1.1\textwidth}}{\small{\textbf{Notes. }The rates shown assume $f_{\rm esc}=1$ and are estimated for the following absorption lines: C-I: 166~nm. C-II: 134~nm. O-I: 130~nm. Na-I: 589~nm. S-I: 181~nm. S-II: 126~nm. S-III: 119~nm. K-I: 767~nm. Each line was selected for having the highest available cross section on the range 100--1800~nm where HST is sensitive. Only species which have absorption lines of sufficiently high cross-section (e.g. $\sigma\geq10^{-16}$~cm$^2$) to be detected with reasonable outgassing rates are included. Absorption cross sections $\sigma$ were computed using \texttt{Cthulhu} \citep{Cthulhu2024JOSS....9.6894A} and binned down to spectral resolution comparable to HST COS, STIS, and WFC3 instruments. \textbf{For wavelengths shorter than $300$~nm, we bin every $0.1$~\AA\,to emulate HST COS and STIS Echelle observations. At wavelengths longer than 300~nm, we bin every 2~nm to emulate HST STIS grating and WFC3 grism observations.} The linelists supplied to \texttt{Cthulhu} were sourced from VALD-3 \citep{VALD}, which relied on data from \cite{INTP}, \cite{MSb}, \cite{NIST10}, \cite{K04},
\cite{K12}, \cite{BPM}, \cite{GUES}, \cite{KP}, 
\cite{LN}, \cite{WSM}, \cite{LWa}, \cite{BQZ}, and \cite{ZCBS}. We also present the total mass loss rate summed across all species as well as the maximum expected torus quasi-steady mass. For reference the total mass loss rate observed from Io is $f_{\rm esc}\dot M_{\rm volc}\sim1$~ton~s$^{-1}$ \citep{Dessler1980Icar...44..291D} and the torus mass is $\sim2$~Mt \citep{BagenalDISTRO1980GeoRL...7...41B}.}}
